Boundary value problems and Hardy spaces for elliptic systems with block structure

For elliptic systems with block structure in the upper half-space and t-independent coefficients, we settle the study of boundary value problems by proving compatible well-posedness of Dirichlet, regularity and Neumann problems in optimal ranges of exponents. Prior to this work, only the two-dimensional situation was fully understood. In higher dimensions, partial results for existence in smaller ranges of exponents and for a subclass of such systems had been established. The presented uniqueness results are completely new. We also elucidate optimal ranges for problems with fractional regularity data. Methods use and improve, with some new results, all the machinery developed over the last two decades to study such problems: the Kato square root estimates and Riesz transforms, Hardy spaces associated to operators, off-diagonal estimates, non-tangential estimates and square functions and abstract layer potentials to replace fundamental solutions in the absence of local regularity of solutions. This self-contained monograph provides a comprehensive overview on the field and unifies many earlier results that have been obtained by a variety of methods.

==> sections/head-chapters.tex <==
\section{Preliminaries on function spaces}

The paragraph

\noindent Throughout, we consider $\IC^k$-valued functions for some fixed $k \in \IN$. For simplicity we often drop the dependence of $k$ in the notation and write $\L^2(\R^n) = \L^2(\R^n; \IC^k)$, and so on. On $\R^n$ we abbreviate further $\L^2 = \L^2(\R^n)$. Concerning the dilemma that parts of the literature only treat scalar-valued functions, we agree on using such results for $k>1$ without further notice in the following cases:
\begin{itemize}
	\item splitting into components is immediately clear from the definition (e.g.\ $\L^2(\R^n; \IC^k) \cong \bigotimes_{j=1}^k \L^2(\R^n; \IC)$),
	
	\item proofs are exactly the same except for a systematic replacement of absolute values by Euclidean norms (e.g.\ Calder\'on--Zygmund decompositions or atomic decompositions).
\end{itemize}


should be moved identically to Section 1.9  after the paragraph Gradient... and before the paragraph Exponents as 

\emph{Convention for vector-valued functions.} Throughout this book, we consider $\IC^k$-valued functions for some fixed $k \in \IN$. For simplicity we often drop the dependence of $k$ in the notation and write $\L^2(\R^n) = \L^2(\R^n; \IC^k)$, and so on. On $\R^n$ we abbreviate further $\L^2 = \L^2(\R^n)$. Concerning the dilemma that parts of the literature only treat scalar-valued functions, we agree on using such results for $k>1$ without further notice in the following cases:
\begin{itemize}
	\item splitting into components is immediately clear from the definition (e.g.\ $\L^2(\R^n; \IC^k) \cong \bigotimes_{j=1}^k \L^2(\R^n; \IC)$),
	
	\item proofs are exactly the same except for a systematic replacement of absolute values by Euclidean norms (e.g.\ Calder\'on--Zygmund decompositions or atomic decompositions).
\end{itemize}

The sentence

The reader can consult this section to find all necessary background whenever new function spaces pop later on in the text.

should be modified  as follows as  header of Chapter 2 

The reader will find in this chapter all necessary background on function spaces used  in the monograph.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries on operator theory}




Add 

We introduce here the elliptic operators used in this monograph and recall their main properties in $L^2$ settings. We also recall material on (bi)sectorial operators and their holomorphic functional calculus.
A particularly useful.... 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\texorpdfstring{$\H^p - \H^q$}{Hp - Hq} bounded families}




One modification: page 43, line 3:  change section to chapter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conservation properties}


No change

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The four critical numbers}

Add

We define four numbers that rule the functional calculus properties of our elliptic operators and that will help describing the ranges of well-posedness of the boundary value problems. 

\subsection{Definition of the critical numbers}

We introduce....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Riesz transform estimates: Part I}

Add

In this chapter, we  characterize the range of $p$ for  $L^p$ boundedness of Riesz transforms $\nabla_x L^{-1/2}$. 

\subsection{Statement of the result}

 We introduce....
 
 [Remark. page 76, line 25: change section to chapter; page 76, line 26: change Sect. to Chapter]
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \section{Operator-adapted spaces} 

One modification: page 87, line 19, change  Sect. to Chapter 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Identification of adapted Hardy spaces}

It is crucial that Figure 9.1 appears as in the submitted version (ie squeezed between lines 6 and  7).


One modification: page 113, line 3:  change section to chapter 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{A digression: $\H^\infty$-calculus and analyticity}

One modification: page 143, line 4: change section to chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Riesz transform estimates: Part II}

No change
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Critical numbers for Poisson and heat semigroups}

Add

In this chapter, we show that the critical numbers are intrinsic in the sense that one could have used other families of functions of $L$ than resolvents to define them, namely the Poisson semigroups, or heat semigroups in the case where  $a=1$. 

\subsection{Definitions and statements}

 For the applications....
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \section{\texorpdfstring{$\L^p$}{Lp} boundedness of the Hodge projector}

Add

In this chapter, we discuss the boundedness properties on $L^p$ of the Hodge projector associated to  $L_{0}$ (that is, in the case where $a=1$). We obtain a characterization of the range of $p$ where this holds 
 
\subsection{Setup and definitions}

Let $p\in (1,\infty)$....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Critical numbers and kernel bounds}

One modification: page 171, line 3, change section to chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Comparison with the Auscher--Stahlhut interval}

One modification: page 187, line 7,  change Sect. to Chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Basic properties of weak solutions}

One modification: page 191, line 7, change section to chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Existence in \texorpdfstring{$\H^p$}{Hp} Dirichlet and Regularity problems}

One modification: page 199, line 4, change section to chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Existence in the Dirichlet problems with \texorpdfstring{$\Lamdot^\alpha$}{Hölder}-data}

one modification: page 215, line 9, change section to chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Existence in Dirichlet problems with fractional regularity data}

One modification: page 239, line 4, change section to chapter. Add a comma after chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Single layer operators for \texorpdfstring{$\Le$}{L} and estimates for \texorpdfstring{$\Le^{-1}$}{L}}

Modifications on page 255, line 4 change section to chapter (twice)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Uniqueness in regularity and Dirichlet problems}

Page 261, line 4 should read: This chapter complements Chapters 17... instead of this section complements Sect. 17...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Neumann problem}

No change

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Non-tangential maximal functions and traces}

One modification: page 289, line 4, change section to chapter and add a comma after chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The \texorpdfstring{$\L^p$}{Lp}-realization of a sectorial operator in \texorpdfstring{$\L^2$}{L2}}

No change


==> sections/multiplicative_perturbation.tex <==
\section{Multiplicative perturbation of real operators}
\label{sec: multiplicative perturbartion of real operators}

\noindent It is tempting to follow further along the lines of Corollary~\ref{cor: q+ indepdendent of a} and compare the critical numbers for $L$ with those for\index{second-order operator!$L_0$}
\begin{align*}
L_0 \coloneqq -\div_x d \nabla_x,
\end{align*}
seeing $L$ as a multiplicative perturbation of $L_0$. Of particular interest would be to prove $p_{-}(L) =  p_{-}(L_0) $ as a general fact. 

Using semigroup techniques, Duong and Ouhabaz~\cite{Ouhabaz, Duong-Ouhabaz} have obtained results in the range $p \geq 1$ if $d$ is a $n\times n$  matrix with real valued coefficients (so $m=1$) under the additional assumption that $d$ is symmetric or, more generally, that the sectoriality angle of $L=a^{-1}L_0$ does not exceed $\nicefrac{\pi}{2}$. In fact, they obtain $(p_-(L) \vee 1) = 1$ and $p_+(L) = \infty$ since the semigroup generated by $L$ has a heat kernel with Gaussian decay. 

Our main objective here is to remove both, the restriction to $p \geq 1$ and the one on the sectoriality angle, and to prove that $p_{-}(L) =  p_{-}(L_0) $ holds if $d$ is a $n\times n$ matrix with real valued coefficients.  We shall also characterize $p_{-}(L_0)$ via a regularity property of its heat kernel. We can restrict ourselves to dimensions $n \geq 2$ since in the one-dimensional setting Proposition~\ref{prop: J(L) contains neighborhood of Sobolev conjugates} already gave the best possible conclusion and there is nothing more to say. 



We recall the following prerequisites from standard elliptic theory. 

\begin{prop}
\label{prop: heat kernel}
Assume that $d$ is real-valued and that $m=1$ and $n \geq 2$. The semigroup generated by $(\e^{-t L_0})_{t>0}$ has the following properties.
\begin{enumerate}
	\item $\L^p$-contractivity for every $p\in [1,\infty]$: Whenever $t>0$ and $f \in \L^p \cap \L^2$,
	\begin{align*}
	\|\e^{-t^2 L_0}f \|_p \leq \|f\|_p.
	\end{align*}
	\item Heat kernel bounds: Whenever $t>0$ and $f \in \L^p \cap \L^2$, then $\e^{-t^2 L_0}f$ is given by a kernel
	\begin{align*}
	\qquad \e^{-t^2 L_0}f(x) = \int_{\R^n} K_t^{(L_0)}(x,y)f(y) \, d y \quad(\text{a.e. } x \in \R^n)
	\end{align*}
	that is measurable in all variables, non-negative, and satisfies for some constants $C, c > 0$ and $\eta_0 \in (0,1]$ that depend on dimensions and ellipticity
	\begin{align*}
	0 \leq K_t^{(L_0)}(x,y) \leq C t^{-n} \e^{-c \frac{|x-y|^2}{t^2}}
	\end{align*}
	and
	\begin{align*}
	\qquad \quad |K_t^{(L_0)}&(x,y+h)-K_t^{(L_0)}(x,y)| + |K_t^{(L_0)}(x+h,y)-K_t^{(L_0)}(x,y)| \\
	&\leq C t^{-n} \bigg(\frac{|h|}{t+|x-y|}\bigg)^{\eta_0} \e^{-c \frac{|x-y|^2}{t^2}}
	\end{align*}
	provided that $2|h| \leq |x-y|$. 
\end{enumerate} 
\end{prop}

One reference for the $\L^p$-contractivity is \cite[Thm.~4.9 \& 4.28]{Ouhabaz}. For the heat kernel bounds the reader can refer to \cite[Thm.~3.23]{Aus1996} when $n \geq 3$ and \cite[Thm.~3.5]{AMcT} when $n =2$. Non-negativity of the heat kernel follows from positivity of the semigroup as stated and proved for instance in \cite[Cor.~4.3]{Ouhabaz}.

In virtue of the Laplace transform, heat kernel bounds can be converted into bounds for the resolvent kernel. We reproduce the argument since less common variants will be needed in the further course.

\begin{cor}
\label{cor: Green kernel}
Assume that $d$ is real-valued and that $m=1$ and $n \geq 2$.
\begin{enumerate}
	\item Let $p\in [1,\infty]$. Whenever $t>0$ and $f \in \L^p \cap \L^2$,
	\begin{align*}
	\|(1+t^2 L_0)^{-1} f \|_p \leq \|f\|_p.
	\end{align*}
	\item For $t>0$ the operator $(1+t^2 L_0)^{-1}$ is given by a non-negative kernel $G_t^{(L_0)}$ that satisfies, for some constants $C, c > 0$ that depend on dimensions and ellipticity and the same $\eta_0$ as in Proposition~\ref{prop: heat kernel}, the following bounds:
	\begin{align*}
	|G_t^{(L_0)}(x,y)| \leq C t^{-n} \bigg(\frac{|x-y|}{t}\bigg)^{2-n} \e^{-c \frac{|x-y|}{t}},
	\end{align*}
	and
	\begin{align*}
	\qquad \quad |G_t^{(L_0)}&(x,y+h)-G_t^{(L_0)}(x,y)| + |G_t^{(L_0)}(x+h,y)-G_t^{(L_0)}(x,y)| \\
	&\leq C t^{-n} \bigg(\frac{|h|}{|x-y|}\bigg)^{\eta_0}  \bigg(\frac{|x-y|}{t}\bigg)^{2-n} \e^{-c \frac{|x-y|}{t}},
	\end{align*}
	provided that $2|h| \leq |x-y|$, where in the first estimate the power function $|\cdot|^{2-n}$ is replaced by $|\ln(\cdot)|+1$ when $n=2$.
\end{enumerate} 
\end{cor}

\begin{proof}
By the functional calculus for $L_0$ we have for $t>0$ and $f \in \L^2$,
\begin{align*}
(1+t^2 L_0)^{-1} f = \int_0^\infty \e^{-s} \e^{-st^2 L_0}f \, \d s.
\end{align*}
Hence, (i) is a consequence of (i) in Proposition~\ref{prop: heat kernel} and on the level of kernels,
\begin{align}
\label{eq1: Green kernel}
G_t^{(L_0)}(x,y) = \int_0^\infty \e^{-s} K_{s^{1/2}t}^{(L_0)}(x,y) \, \d s.
\end{align}
Since $ K_{s^{1/2}t}^{(L_0)}$ is non-negative, so is $G_t^{(L_0)}$. To get the bounds for $G_t^{(L_0)}$, we use (ii) in Proposition~\ref{prop: heat kernel} to give
\begin{align}
\label{eq2: Green kernel}
\begin{split}
|G_t^{(L_0)}(x,y)| 
&\leq C t^{-n} \int_0^\infty s^{-\frac{n}{2}} \e^{-s} \e^{-c \frac{|x-y|^2}{st^2}} \, \d s \\
&\leq C t^{-n} \e^{-\sqrt{c}A} \int_0^\infty s^{-\frac{n}{2}} \e^{-\frac{s}{2}} \e^{-\frac{c A^2}{2s}} \, \d s,
\end{split}
\end{align}
where $A \coloneqq \nicefrac{|x-y|}{t}$ and we have used the elementary inequality $\nicefrac{s}{2} + \nicefrac{cA^2}{(2s)} \geq \sqrt{c}A$ in the second step. We split the integral at $s=A^2$ and substitute $u = \nicefrac{A^2}{s}$ for small $s$ to obtain
\begin{align*}
|G_t^{(L_0)}(x,y)| 
&\leq C t^{-n} \e^{-\sqrt{c}A}  \bigg(\int_1^\infty A^{2-n} u^{\frac{n}{2}-1} \e^{-\frac{c}{2}u } \, \d u + \int_{A^2}^\infty s^{-\frac{n}{s}} \e^{-\frac{s}{2}} \, \d s \bigg),
\end{align*}
which has the required behavior as a function of $A$. 

The argument for the H\"older continuity of $G_t^{(L_0)}$ is exactly the same. When integrating the analogous bound for $K_t^{(L_0)}$ as in \eqref{eq1: Green kernel}, we generously bound $\nicefrac{|h|}{(t+|x-y|)}$ by $\nicefrac{|h|}{t}$.
\end{proof}

The bounds for the resolvent kernel imply an upper estimate for $p_-(L_0)$. As it turns out, only the H\"older regularity of $G_t^{(L_0)}$ in the second variable is needed in the argument. Since $G_t^{(L_0)}(x,y) = G_t^{(L_0^*)}(y,x)$, this corresponds to H\"older regularity of solutions to the adjoint equation 
\begin{align*}
	(1+t^2 L_0^*)u = f
\end{align*} 
and we introduce the following critical number\index{critical numbers!for heat kernel regularity ($\eta_0(L_0)$)}. 

\begin{defn}
\label{def: critical number Holder regularity}
Denote by $\eta_0(L_0^*)$ the supremum of all exponents $\eta_0 \in (0,1]$ such that the H\"older estimate in the second variable  in Corollary~\ref{cor: Green kernel}.(ii) holds with exponent $\eta_0$.
\end{defn}

\begin{lem}
\label{lem:real operators} 
Assume that $d$ is real-valued and that $m=1$ and $n \geq 2$. Then $p_-(L_0) \leq \nicefrac{n}{(n+\eta_0(L_0^*))}$.
\end{lem}


\begin{proof} 
We have to show that for fixed $\eta_0 \in (0, \eta_0(L_0^*))$ and $p \in (\nicefrac{n}{(n+\eta_0)},1)$ the family $(1+t^2L_0)^{-1}$ is $\H^p$-bounded. It suffices to establish for some $C, \eps > 0$ the molecular bounds 
\begin{align}
\label{eq1: real operators}
\|(1+t^2L_0)^{-1}m\|_{\L^2(C_j(B))} \leq C (2^{j} r(B))^{\frac{n}{2}-\frac{n}{p}} 2^{-\eps j} \quad (j \geq 1),
\end{align}
whenever $t>0$ and $m$ is an $\L^2$-atom for $\H^p$ associated with a ball $B$. Indeed, since $(1+t^2L_0)^{-1}m$ has integral zero by Corollary~\ref{cor: conservation}, we can first use Lemma~\ref{lem: Taibleson-Weiss} to get a uniform $\H^p$-bound and then conclude by the ($\L^2$-convergent) atomic decomposition.
 
For $j = 1$ we have as required
\begin{align*}
\|(1+t^2L_0)^{-1}m\|_{\L^2(C_1(B))}
\leq \|m\|_2 \leq r(B)^{\frac{n}{2}-\frac{n}{p}}.
\end{align*}
For $j \geq 2$ we use the mean value property of $m$ to write
\begin{align*}
(1+t^2 L_0)^{-1} m(x) = \int_{B} (G_t^{(L_0)}(x,y)-G_t^{(L_0)}(x,y_B))m(y) \, \d y
\end{align*}
with $y_B$ the center of $B$ and obtain for $x \in C_j(B)$ that
\begin{align*}
|(1+t^2 L_0)^{-1} m(x)| 
&\leq C t^{-n} 2^{-j \eta_0} \bigg(\frac{2^{j-1} r(B)}{t}\bigg)^{2-n} \e^{-c \frac{2^{j-1} r(B)}{t}} \|m\|_1 \\
&\leq C C' t^{-n} 2^{-j \eta_0} \bigg(\frac{2^{j-1} r(B)}{t}\bigg)^{-n} r(B)^{n-\frac{n}{p}},
\end{align*}
where $C' \coloneqq \sup_{s>0} s^2 \e^{-cs}$. On the right-hand side $t$ cancels. Sorting powers of $2^j$ and $r(B)$ and integrating in $x$ gives \eqref{eq1: real operators} with $\eps \coloneqq \nicefrac{n}{p}-n-\eta_0$. Now $\eps > 0$ is equivalent to $p> \nicefrac{n}{(n+\eta_0)}$, which we have assumed. 
\end{proof}

When perturbing $L_0$ to $L$ it is convenient to view $a$ as a perturbation of $1$ in the following sense.

\begin{lem}
\label{lem: accr-representation}
There are $\tau \ > 0$ and $b \in \L^\infty(\R^n;\Lop(\IC^m))$ with $\|b\|_\infty  < 1$ such that
\begin{align*}
	a= \tau(1-b).
\end{align*}
One choice is $\tau = \lambda^{-1} \|a\|_\infty^2$, in which case $\|b\|_\infty \leq \sqrt{1 - \lambda^2 \|a\|_\infty^{-2}}$.
\end{lem}

\begin{proof}
We let $\tau \coloneqq \lambda^{-1} \|a\|_\infty^{-2}$ as suggested and hence we have to take $b \coloneqq 1- \tau^{-1}a$. If $\xi  \in  \IC^m$ is normalized to $|\xi| = 1$, then 
\begin{align*}
	|b(x)\xi|^2 
	&= 1 + \tau^{-2}|a(x) \xi |^2 - 2 \tau^{-1} \Re \langle a(x) \xi, \xi \rangle \\
	&\leq 1 + \tau^{2} \|a\|_\infty^2 - 2 \tau^{-1} \lambda \\
	&= 1 - \lambda^2 \|a\|_\infty^{-2}. \qedhere
\end{align*}
\end{proof}

We obtain a simple identity relating resolvents of $L$ and $L_0$ that will be our key tool in the following.

\begin{lem}
\label{lem: Neumann series}
If $a=\tau(1-b)$ is a decomposition as in Lemma~\ref{lem: accr-representation}, then as operators on $\L^2$,
\begin{align*}
	(1+t^2L)^{-1} = \tfrac{1}{\tau} (1- (1+ \tfrac{t^2}{\tau}L_0)^{-1}b)^{-1}(1+ \tfrac{t^2}{\tau}L_0)^{-1}a \quad (t>0),
\end{align*}
where the first operator on the right-hand side is given by an absolutely convergent Neumann series.
\end{lem}

\begin{proof}
The operator  $(1+ \nicefrac{t^2}{\tau}L_0)^{-1}$ is a contraction on $\L^2$ since $L_0$ is maximal accretive~\cite[Thm.~VI.2.1]{Kato}. Since $\|b\|_\infty < 1$, we can invert $1- (1+ \nicefrac{t^2}{\tau}L_0)^{-1}b$ by a Neumann series. The identity in question then follows directly:
\begin{align*}
(1+t^2L)^{-1} 
&= (a^{-1}(a+t^2L_0))^{-1}  \\
&= (1-b+\tfrac{t^2}{\tau}L_0)^{-1}(1-b)\\
&= \tfrac{1}{\tau} (1- (1+ \tfrac{t^2}{\tau}L_0)^{-1}b)^{-1}(1+ \tfrac{t^2}{\tau}L_0)^{-1}a. \qedhere
\end{align*}
\end{proof}

We come to a first perturbation result. 

\begin{prop}
\label{prop:dreal baby}
Assume that $d$ is real-valued and that $m=1$ and $n \geq 2$. It follows that
\begin{align*}
	p_-(L) = p_-(L_0)  \quad \text{and} \quad p_+(L) = p_+(L_0) = \infty.
\end{align*}
\end{prop}

\begin{proof}
We proceed in three steps.

\medskip

\noindent \emph{Step~1:  $((1+t^2L)^{-1})_{t>0}$ is $\L^p$-bounded for $1\le p\le \infty$.} We decompose $a=\tau(1-b)$ according to Lemma~\ref{lem: accr-representation} and use the identity \begin{align*}
	(1+t^2L)^{-1} = \tfrac{1}{\tau} \bigg(\sum_{j=0}^\infty \big((1+\tfrac{t^2}{\tau}L_0)^{-1}b \big)^j \bigg) (1+ \tfrac{t^2}{\tau}L_0)^{-1}a 
\end{align*}
from Lemma~\ref{lem: Neumann series}. As $(1+t^2L_0)^{-1}$ extends to a contraction on $\L^p$ by Corollary~\ref{cor: Green kernel}, the  Neumann series, call it $U(t)$,  is also bounded on $\L^p$ with norm controlled by $(1-\|b\|_\infty)^{-1}$. This shows that $(1+t^2L)^{-1}$ is $\L^p$-bounded with bound $\tau^{-1} \|a\|_\infty (1-\|b\|_\infty)^{-1}$. Thus, $p_-(L) \leq 1$ and $p_+(L) = p_+(L_0) = \infty$.

\medskip

\noindent \emph{Step~2: $p_-(L)\le p_-(L_0) $.}  From Lemma~\ref{lem:real operators} we already know that $p_-(L_0)<1$. Hence, it suffices to pick $p_-(L_0)<p< 1$ and show that $T(t) \coloneqq a(1+t^2L)^{-1}a^{-1}$ is  $\H^p$-bounded. To this end, we apply Lemma~\ref{lem: OD Hardy implies boundedness} as follows. 

Let $p_-(L_0)<\rho<p$ and set $q \coloneqq \rho^*$. By a Sobolev embedding and since $p_-(L_0) = q_-(L_0)$, we find
\begin{align*}
\|(1+t^2L_0)^{-1}f\|_q \lesssim \|\nabla_x (1+t^2L_0)^{-1}f \|_{\H^\rho} \lesssim t^{-1} \|f\|_{\H^\rho},
\end{align*}
whenever $f \in \H^\rho \cap \L^2$ and $t>0$. This means that $(1+t^2 L_0)^{-1}$ is $\H^\rho-\L^q$-bounded. In Step~1 we have seen that
\begin{align*}
	T(t)f= \tfrac{1}{\tau} aU(t)(1+\tfrac{t^2}{\tau}L_0)^{-1}f,
\end{align*}
where $U(t)$ is $\L^q$-bounded. Hence, $T(t)$ is $\H^\rho-\L^q$-bounded as well. Second, $T(t)$ has $\L^q$ off-diagonal bounds of arbitrary order by interpolation from the ones on $\L^2$ and the uniform $\L^r$-bounds from Step~1 for some $r \in (1,q)$. Third, the cancellation property $\int_{\R^n}T(t)f\, \d x=0$ for compactly supported $\L^2$-functions with integral $0$ is granted from Corollary~\ref{cor: conservation}. We conclude that $T(t)$ is $\H^p$-bounded.

\medskip

\noindent \emph{Step~3:  $p_-(L_0)\le p_-(L) $.} This time we let $p_-(L)<p< 1$ and use Lemma~\ref{lem: OD Hardy implies boundedness} to prove that $T(t) \coloneqq (1+t^2L_0)^{-1}$ is  $\H^p$-bounded.

Letting $p_-(L)<\rho<p$ and $q \coloneqq \rho^*$, we obtain as before that $(1+t^2 L)^{-1}a^{-1}$ is $\H^\rho-\L^q$-bounded. According to Lemma~\ref{lem: Neumann series} with $t \tau^{1/2}$ instead of $t$, we have
\begin{align*}
\tau (1- (1+ t^2 L_0)^{-1}b) (1+t^2 \tau L)^{-1}a^{-1} = 	T(t).
\end{align*}
The first factor on the left is $\L^q$-bounded by Corollary~\ref{cor: Green kernel}. Thus, $T(t)$ is $\H^\rho-\L^q$-bounded as well. The other assumptions of Lemma~\ref{lem: OD Hardy implies boundedness} follow as in Step~2 from the general theory since $L_0$ is a particular operator in the same class as $L$.
\end{proof}

Next, we show that regularity and decay of the resolvent kernel are preserved under multiplicative perturbations. Step~2 of our proof simplifies the corresponding argument in~\cite[Thm.~2.2]{Duong-Ouhabaz}.\index{Resolvent kernel bounds!for perturbations of real operators}

\begin{thm} 
\label{thm:pointwise estimates} 
Assume that $d$ is real-valued and that $m=1$ and $n \geq 2$. The operators $(1+t^2L)^{-1}a^{-1}$, $t>0$, are given by complex-valued kernels with the same type of pointwise bounds and regularity estimates as for $(1+t^2L_0)^{-1}$ in Corollary~\ref{cor: Green kernel}.(ii). The regularity exponent can be any $\eta \in (0, \eta_0)$ and the constants $C,c$ depend on $\eta$, ellipticity and dimensions.
\end{thm}


\begin{proof}  
The argument is organized in four steps.

\medskip

\noindent \emph{Step 1: High resolvent powers}. From the size estimate of the kernel in Corollary~\ref{cor: Green kernel}.(ii) and Young's convolution inequality, $(1+t^2L_0)^{-1}$, $t>0$, is $\L^p -\L^q$-bounded whenever $1\le p \leq q\le \infty$ satisfy $\nicefrac{1}{p}-\nicefrac{1}{q} < \nicefrac{2}{n}$. By Corollary~\ref{cor: Green kernel}.(i) the same operator is $\L^p$-bounded with bound at most $1$. Hence, the identity in Lemma~\ref{lem: Neumann series} continues to hold in $\L^p$ and implies the same $\L^p-\L^q$-bounds hold for $(1+t^2L)^{-1}$.

In particular, there exists an integer $\beta > \nicefrac{n}{2}$ that depends on $n$ such that $(1+t^2L)^{-\beta}$ is $\L^1 - \L^\infty$-bounded with a bound $C t^{-n}$, where $C$ depends on dimension and ellipticity. By the Dunford--Pettis theorem~\cite[Thm.~1.3]{Arendt-Bukhvalov}\index{Theorem!Dunford--Pettis} it follows that $(1+t^2L)^{-\beta}$ is given by a measurable kernel $H_t^{(L)}$ with pointwise bounds
\begin{align}
\label{eq1:pointwise estimates}
|H_t^{(L)}(x,y)| \leq C  t^{-n}  \quad (x,y \in \R^n).
\end{align}
For $L_0$ in place of $L$ we can use the formula (a Calderón reproducing formula for the invertible sectorial operator $1+t^2 L_0$),
\begin{align}
\label{eq4:pointwise estimates}
(1+t^2 L_0)^{-\beta} = \frac{1}{\beta!} \int_0^\infty s^{\beta-1} \e^{-s} \e^{-s t^2 L_0} \, \d s
\end{align}
to get from the size of the non-negative heat kernel in Proposition~\ref{prop: heat kernel} the pointwise bound
\begin{align}
\label{eq2:pointwise estimates}
H_t^{(L_0)}(x,y) \leq C t^{-n} \e^{- c \frac{|x-y|}{t}} \quad (x,y \in \R^n).
\end{align}
The calculation is the same as in \eqref{eq2: Green kernel} but we can drop the term $\e^{-cA^2/(2s)} \leq 1$ directly since $\beta > \nicefrac{n}{2}$. The constants $C,c>0$ depend again on dimension and ellipticity.

\noindent

\noindent \emph{Step 2: Pointwise domination of $H_t^{(L)}$ by $H_t^{(L_0)}$.} For the rest of this step we let $t>0$ and $f \in \L^2$. As usual, we decompose $a=\tau(1-b)$ according to Lemma~\ref{lem: accr-representation} and use the identity \begin{align*}
	(1+t^2L)^{-1} f = \tfrac{1}{\tau} \sum_{j=0}^\infty \big((1+\tfrac{t^2}{\tau}L_0)^{-1}b \big)^j (1+ \tfrac{t^2}{\tau}L_0)^{-1}a f
\end{align*}
from Lemma~\ref{lem: Neumann series}. Since the resolvents of $L_0$ are $\L^\infty$-contractive and given by a non-negative kernel (Corollary~\ref{cor: Green kernel}), we have a.e.\ on $\R^n$ the pointwise estimate
\begin{align*}
	|(1+\tfrac{t^2}{\tau}L_0)^{-1}b f| 
	\leq \|b\|_\infty (1+\tfrac{t^2}{\tau}L_0)^{-1}  |f| 
	\leq \|b\|_\infty  |f|.
\end{align*}
Iterating this estimate, we first obtain from the Neumann series that
\begin{align}
\label{eq5:pointwise estimates}
\begin{split}
	|(1+t^2L)^{-1} f | 
	&\leq \tfrac{1}{\tau(1-\|b\|_\infty)}  |(1+\tfrac{t^2}{\tau}L_0)^{-1} af| \\
	&\leq \tfrac{\|a\|_\infty}{\tau(1-\|b\|_\infty)}  (1+\tfrac{t^2}{\tau}L_0)^{-1}  |f| ,
\end{split}
\end{align}
which when being iterated itself $\beta$-times, where $\beta$ is as in Step~1, leads us to
\begin{align*}
	|(1+t^2 L)^{-\beta} f| \leq ( \tfrac{\|a\|_\infty}{\tau(1-\|b\|_\infty)})^\beta  (1+ \tfrac{t^2}{\tau} L_0)^{-\beta} |f|.
\end{align*}
Applying the pointwise bound to characteristic functions $f$ of sets with finite measure yields the pointwise comparability of the corresponding kernels:
\begin{align}
\label{eq6:pointwise estimate}
	|H_t^{(L)}(x,y)| \leq ( \tfrac{\|a\|_\infty}{\tau(1-\|b\|_\infty)})^\beta  H_{t\tau^{-1/2}}^{(L_0)}(x,y)  \quad (x,y \in \R^n).
\end{align}

\noindent \emph{Step 3: Size of the kernel for $(1+t^2L)^{-1}a^{-1}$}. Combining \eqref{eq2:pointwise estimates} and \eqref{eq6:pointwise estimate}, we find $C',c' > 0$ that depend on dimensions and ellipticity, such that 
\begin{align}
	\label{eq3:pointwise estimates}
	|H_t^{(L)}(x,y)| \leq C' t^{-n} \e^{- c' \frac{|x-y|}{t}} \quad (x,y \in \R^n).
\end{align}
By the formula
\begin{align*}
(1+t^2 L)^{-1}(a^{-1}f) = (\beta-1) \int_0^\infty (1+u+t^2u L)^{-\beta}(a^{-1}f) \, \d u,
\end{align*}
which follows by applying $(1+t^2L)^{-1}$ to both sides of \eqref{eq: resolution of resolvents through high powers}, we see that $(1+t^2L)^{-1} a^{-1}$ is given by a kernel with bound
\begin{align*}
|G_t^{(L)}(x,y)| 
&\leq C' t^{-n} \int_0^\infty (1+u)^{-\beta} (1+\tfrac{1}{u})^{\frac{n}{2}} \e^{-c'\frac{|x-y|}{t}(1+\frac{1}{u})^{\nicefrac{1}{2}}} \, \d u \\
&\leq C' t^{-n} \int_0^\infty (1+\tfrac{1}{u})^{\frac{n}{2}-2} \e^{-c' \frac{|x-y|}{t}(1+\frac{1}{u})^{\nicefrac{1}{2}}} \, \frac{\d u}{u^2} \\
&= C' t^{-n} \bigg(\frac{|x-y|}{t}\bigg)^{2-n} \int_{\frac{|x-y|^2}{t^2}}^\infty v^{\frac{n}{2}-2} \e^{-c' v^{\nicefrac{1}{2}}} \, \d v.
\end{align*}
Now, we can read off the required decay
\begin{align*}
|G_t^{(L)}(x,y)| \leq C'' t^{-n} \bigg(\frac{|x-y|}{t}\bigg)^{2-n} \e^{-c''\frac{|x-y|}{t}}
\end{align*}
with the usual modification in dimension $n = 2$.

\medskip

\noindent \emph{Step 4: H\"older continuity of the kernel}. Let $\eta \in (0,\eta_0)$. We set $\rho \coloneqq \nicefrac{n}{(n+\eta)}$ and $q \coloneqq \rho^*$. By Step~1 there is $\beta \geq 2$ such that  $(1+t^2 L)^{-\beta+1}$, $t>0$, is $\L^1 - \L^{q'}$-bounded. By Proposition~\ref{prop:dreal baby} and Lemma~\ref{lem:real operators} applied to the adjoint, we get that $\rho > p_-((a^*)^{-1} L_0^*)$. As in Step~2 of the proof of Proposition~\ref{prop:dreal baby} we get that $(1+t^2 (a^*)^{-1} L_0^*)^{-1}$ is $(a^*)^{-1} \H^\rho - \L^q$-bounded and by duality,
\begin{align*}
\|(1+t^2 L)^{-1}\|_{\L^{q'} \to \Lamdot^\eta} \leq C t^{\frac{n}{q} -n -\eta},
\end{align*}
in the sense that there is an extension  with the respective operator norm bound. Here, $C$ depends on dimensions and ellipticity. Altogether, 
\begin{align*}
\|(1+t^2 L)^{-\beta}\|_{\L^1 \to \Lamdot^\eta} \leq C t^{-n -\eta}.
\end{align*}
Now, let $h \in \R^n$ and $\tau_h$ the translation operator $(\tau_hf)(x) \coloneqq f(x+h)$. The previous bound implies with the same constant $C$,
\begin{align*}
\|(\tau_h-1)(1+t^2 L)^{-\beta}\|_{\L^1 \to \L^\infty} \leq C t^{-n-\eta} |h|^\eta.
\end{align*}
The kernel of $(\tau_h-1)(1+t^2 L)^{-\beta}$ is $H_t^{(L)}(\cdot+h,\cdot) - H_t^{(L)}(\cdot,\cdot)$. Hence, we obtain almost everywhere that
\begin{align*}
|H_t^{(L)}(x+h,y) - H_t^{(L)}(x,y)| \leq C t^{-n-\eta} |h|^\eta.
\end{align*}
This works for every $\eta \in (0,\eta_0)$ and $C$ depends on $\eta$, $\eta_0$, ellipticity and dimension. If in addition $2|h| \leq |x-y|$, then by \eqref{eq3:pointwise estimates} and the triangle inequality
\begin{align*}
|H_t^{(L)}(x+h,y) - H_t^{(L)}(x,y)|  \leq 2 C't^{-n}\e^{-\frac{c'}{2} \frac{|x-y|}{t}}.
\end{align*}
Interpolating between these bounds yields for any $\eta \in (0,\eta_0)$ new constants $C',c' > 0$ depending on ellipticity, dimension, $\eta$ and $\eta_0$, such that
\begin{align*}
|H_t^{(L)}(x+h,y) - H_t^{(L)}(x,y)| 
&\leq C' |h|^\eta t^{-n-\eta} \e^{-c'\frac{|x-y|}{t}}
\end{align*}
for $2|h| \leq |x-y|$. This is the substitute for \eqref{eq3:pointwise estimates} and we can follow Step~3 to get
\begin{align}
\label{eq7:pointwise estimates}
\begin{split}
&\quad |G_t^{(L)}(x+h,y)-G_t^{(L)}(x,y)|\\
&\leq C'' t^{-n} \bigg(\frac{|h|}{|x-y|}\bigg)^{\eta}  \bigg(\frac{|x-y|}{t}\bigg)^{2-n} \e^{-c'' \frac{|x-y|}{t}}.
\end{split}
\end{align}
Of course the same type of regularity estimate then holds for the kernel $G_t^{(L)}(x,y) a^{-1}(y)$ of $(1+t^2 L)^{-1} a^{-1}$.

The corresponding regularity estimate in the $y$-variable follows by considering the adjoint kernel $G_t^{(L)}(y,x) a^{-1}(x)$, which corresponds to the operator $(1+t^2 (a^*)^{-1} L_0^*)^{-1} (a^*)^{-1}$.
\end{proof}

\begin{rem}
\label{rem:dreal}
The proof above shows slightly more: The H\"older estimate \eqref{eq7:pointwise estimates} holds for all exponents $\eta \in (0,1)$ such that $\nicefrac{n}{n+\eta} > p_-(L_0^*)$ and the corresponding estimate in the second variable holds provided that $\nicefrac{n}{n+\eta} > p_-(L_0)$. Indeed, we have used the definition of $\eta_0$ only in Step~4 in order to guarantee (via Proposition~\ref{prop:dreal baby} and Lemma~\ref{lem:real operators}) that precisely these inequalities hold.
\end{rem}

Summarizing our findings, we obtain a complete description of the critical numbers of multiplicative perturbations of real operators. The assumptions that $m=1$ and $d$ is real-valued lead to improvements compared to the general theory for all but $q_+(L)$, compare with Remark~\ref{rem: Frehse}. We recall that the critical number $\eta_0(L_0^*)$ has been introduced in Definition~\ref{def: critical number Holder regularity}.

\begin{thm}
\label{thm:dreal} 
Assume that $d$ is real-valued and that $m=1$ and $n \geq 2$. It follows that\index{critical numbers!for perturbations of real operators} 
\begin{enumerate}
	\item $p_{-}(L) = p_{-}(L_0) =\frac{n}{n+\eta_0(L_0^*)}$,
	\item $q_{-}(L) =  q_{-}(L_0) = \frac{n}{n+\eta_0(L_0^*)}$,
	\item $p_{+}(L) = p_+(L_0) = \infty$,
	\item $q_{+}(L) =  q_{+}(L_0)$.
\end{enumerate}
\end{thm}

\begin{proof}
Parts (iii) and (iv) have been obtained in Proposition~\ref{prop:dreal baby} and Corollary \ref{cor: q+ indepdendent of a}, respectively. Moreover, (ii) reduces to (i)  by Theorem~\ref{thm: standard relation J(L) and N(L)}. Proposition~\ref{prop:dreal baby} also yields $p_{-}(L) = p_{-}(L_0)$. Finally, $\nicefrac{n}{n+\eta_0(L_0^*)} \leq p_-(L_0)$ follows from Remark~\ref{rem:dreal} in the special case that $L=L_0$, whereas the opposite estimate has already been obtained in Lemma~\ref{lem:real operators}.
\end{proof}

We close this section with kernel estimates in the special case of $L=-a^{-1}\Delta_x$, using a much simpler method than the original proof in \cite{McN}. Let us mention that for this result there are no restrictions on $m$ and $n$.%\index{Green kernel bounds!for perturbations of the Laplacian}\index{Theorem!McIntosh--Nahmod's} 

\begin{prop} 
%\label{prop: pointwise estimates} 
For all integers $\beta> \nicefrac{n}{2}+2$ the following properties hold for the kernel $G_t(x,y)$ of the resolvents $(1-t^2a^{-1}\Delta_x)^{-\beta} a^{-1}$ .
\begin{enumerate}
\item There are $C,c>0$, depending on ellipticity, dimensions and $\beta$, such that one has for for all $t>0$ and $x,y\in \R^n$, 
\begin{align*}
\qquad |G_t(x,y)|+ |t\nabla_x G_t(x,y)|+ |t\nabla_y G_t(x,y)|
\\
+  |t^2\nabla_x \nabla_y G_t(x,y)| \le Ct^{-n}\e^{-\frac{c|x-y|}{t}}.
\end{align*}
\item For all $\eta \in (0,1)$, the kernels
\begin{align*}
\qquad t\nabla_x G_t(x,y), \quad  t\nabla_y G_t(x,y), \quad t^2\nabla_x \nabla_y G_t(x,y)
\end{align*}
are H\"older continuous in both variables with exponent $\eta$ and norms of the order of $t^{-\eta-n}$.  In particular, 
$G_t \in \C^{1, \eta}(\R^n \times \R^n)$, the space of $\C^1$ functions having H\"older continuous of exponent $\eta$ first order derivatives.
\end{enumerate}
\end{prop}

\begin{proof}
It suffices to prove the properties of $G_t$  for $t=1$ with implicit constants that depend on $a$ only through ellipticity. Indeed, setting $G_t^{(a)}=G_t$, a change of variables yields
\begin{align*}
G_t^{(a)}(x,y) = t^{-n} G_1^{(a_t)}(\tfrac{x}{t}, \tfrac{y}{t}),
\end{align*}
where $a_t(x) \coloneqq a(tx)$ has the same ellipticity constants as $a$. We split the proof into three steps.

\medskip

\noindent{\emph{Step~1: Proof of (ii) and (i) with $c=0$.}} As before, we write $L= a^{-1}L_0$ with $L_0 \coloneqq -\Delta_x$. We use Lemma~\ref{lem: accr-representation} to write $a=\tau(1-b)$ as in the case $m=1$. Since $(1+L_0)^{-1}$ acts as $(1-\Delta_x)^{-1}$ on each component of a $\IC^m$-valued functions, this operator is still $\L^p$-bounded with bound at most $1$. Thus, we can use the Neumann series identity from Lemma~\ref{lem: Neumann series} to obtain for all $1\le p < q\le \infty$ extensions by density with operator norm bounds
\begin{align*}
\| (1+L)^{-1}a^{-1} \|_{\L^p\to\L^q} &\le \frac{1}{\tau(1-\|b\|_\infty)} \| (1+ \tfrac{1}{\tau}L_0)^{-1} \|_{\L^p\to\L^q},\\
\| \Delta_x(1+L)^{-1}a^{-1} \|_{\L^p\to\L^p} &\le 1+\frac{\|1-b\|_\infty}{1-\|b\|_\infty} \| (1+\tfrac{1}{\tau} L_0)^{-1} \|_{\L^p\to\L^p},
\end{align*}
where for the second line we simply write $\Delta_x(1+L)^{-1} = -a+a(1+L)^{-1}$ and then use the first line. 

The operator norm in the first line is controlled for all $p$ and $q$ with $\nicefrac{1}{p}-\nicefrac{1}{q}<\nicefrac{2}{n}$ and this gives $\L^1-\L^\infty$-boundedness of $(1+L)^{-\beta} a^{-1}$ provided that $\beta> \nicefrac{n}{2}$. By the Dunford--Pettis theorem we obtain that $(1+L)^{-\beta} a^{-1}$ is given by a bounded kernel $G=G_1$ and the bound depends only on dimensions and ellipticity.

The operator norm in the second line above is controlled for all $p$. If $1<p<\infty$,  then by the Mihlin multiplier theorem the two estimates imply that $(1+L)^{-1} a^{-1}$ and  $\nabla_x(1+L)^{-1} a^{-1}$ are bounded from $\L^p$ to $\W^{1,p}$. In particular, for $p>n$, we have the inhomogeneous Sobolev embedding $\W^{1,p}\subseteq \Lamdot^\eta \cap \L^\infty$, $\eta=1-\nicefrac{n}{p}$. The same applies with $a^*$ in place of $a$ and by duality $(1+L)^{-1} a^{-1} \div_x$  is bounded from $\L^1$ to $\L^{p'}$. By composition, we obtain that for $\beta > \nicefrac{n}{2} +2$ the operators
\begin{align*}
&\nabla_x(1+L)^{-\beta}a^{-1}, \quad  (1+L)^{-\beta}a^{-1}\div_x, \quad \nabla_x(1+L)^{-\beta} a^{-1}\div_x  
\end{align*}
are bounded from $\L^1$ into $\Lamdot^\eta \cap \L^\infty$. In particular they are bounded from $\L^1$ into $\L^\infty$ and, invoking again the Dunford--Pettis theorem, they correspond to the kernels $\nabla_x G$, $\nabla_y G$, $\nabla_x \nabla_y G$, which therefore are bounded measurable functions. As in Step~4 of the proof of Theorem~\ref{prop: pointwise estimates}, we can then use the mapping properties into $\Lamdot^\eta$ , in order to obtain first H\"older continuity of the kernels in $x$ (with any exponent $\eta \in (0,1)$), uniformly in $y$, and then by duality the same with the roles of $x$ and $y$ reversed. This proves (ii) and (i) with $c=0$.

\medskip

\noindent{\emph{Step~2: Exponential decay for $G$.}} We want to use the argument of Step~2 in the proof of Theorem~\ref{thm:pointwise estimates}. This proof was for $m=1$ but the assumption was only used in order to guarantee that $(1+L_0)^{-1}$ is $\L^\infty$-contractive and given by a non-negative kernel. Here, both assumptions still hold componentwise. Hence, we obtain by said argument, and as a substitute for \eqref{eq5:pointwise estimates}, the pointwise bound
\begin{align*}
	|(1+L)^{-1} f | 
\leq \tfrac{\|a\|_\infty}{\tau(1-\|b\|_\infty)}  (1-\tfrac{1}{\tau}\Delta_x)^{-1}  |f| ,
\end{align*}
for all $f \in \L^2$. Note that on the right-hand side we are using the resolvent of the operator $-\Delta_x$ on scalar-valued $\L^2$. 

Iterating $\beta$-times, we find as before the kernel $G$ of $(1+L)^{-\beta}$ is dominated by the kernel of $(1-  \tau^{-1} \Delta_x)^{-\beta}$. The latter has the required exponential decay, see \eqref{eq2:pointwise estimates}.
\medskip

\noindent{\emph{Step~3: Exponential decay for the other kernels.}} We begin with $\partial_{x_i} G$, where $1 \leq i \leq n$. Let $e_i \in \R^n$ be the $i$-th standard unit vector and let $h>0$. By the fundamental theorem of calculus we have
\begin{align*}
	&\frac{1}{h} (G(x+he_i,y) - G(x,y))  \\
	&=\quad \barint_0^h \partial_{x_i} G(x+s e_i,y) \, \d s \\
	&=\quad \partial_{x_i}G(x,y) + \barint_0^h \partial_{x_i} G(x+s e_i,y) - \partial_{x_i}G(x,y) \, \d s,
\end{align*}
where $x,y \in \R^n$. If  $2|h| \leq |x-y|$, then $|x+h e_i - y| \geq \nicefrac{|x-y|}{2}$ and we get from (i) for $G$ and (ii) for $\nabla_x G$ that
\begin{align*}
	|\partial_{x_i}G(x,y)| \leq \frac{C}{h}\big(\e^{-\frac{c}{2}|x-y|} + \e^{-c|x-y|}\Big) + h^\eta \|\nabla_x G\|_{\Lamdot^\eta}. 
\end{align*}
Since in Step~1 we have already obtained a uniform bound for $\partial_{x_i} G$, it suffices to prove the decay for $|x-y|$ large, say $|x-y| \e^{\frac{c}{4}|x-y|} \geq 2$. This restriction is manufactured such that we can take $h \coloneqq \e^{-\frac{c}{4}|x-y|}$, resulting in the desirable estimate
\begin{align*}
		|\partial_{x_i}G(x,y)| \leq C' \e^{-\frac{\eta c}{4}|x-y|}
\end{align*}
for some new constant $C'$ that depends on $a$ only through ellipticity. This completes the proof for $\nabla_x G$.

The argument above has only used the exponential decay for $G$, the uniform boundedness of $\nabla_x G$ and the $\Lamdot^\eta$-estimate for $\nabla_x G$ in the $x$-variable, in order to give exponential decay for $\nabla_x G$. Thus, it can be repeated \emph{verbatim} for the decay of $\nabla_y G$. Then, replacing $G$ by $\nabla_y G$ gives decay of $\nabla_x \nabla_y G$.
\end{proof}

\begin{rem}
Since $-\Delta_x$ is self-adjoint, the operator $L=-a^{-1}\Delta_x$ is sectorial of angle less than $\omega<\nicefrac{\pi}{2}$, see for instance \cite[Prop.~7.1]{AMcN1}. Hence, $-L$ generates a holomorphic $\C_0$-semigroup on $\L^2$. By extension of (i) and (ii) to complex parameters $e^{i\theta}t^2$ for $\theta \in (-\nicefrac{\pi}{2}+\omega, \nicefrac{\pi}{2}-\omega)$ and a contour integral, one can derive Gaussian kernel bounds for $\e^{-tL}$. This will not be needed in this book. The interested reader can refer to \cite{McN}.
\end{rem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
